ExAD: An Ensemble Approach for Explanation-based Adversarial Detection

Recent research has shown Deep Neural Networks (DNNs) to be vulnerable to adversarial examples that induce desired misclassifications in the models. Such risks impede the application of machine learning in security-sensitive domains. Several defense methods have been proposed against adversarial attacks to detect adversarial examples at test time or to make machine learning models more robust. However, while existing methods are quite effective under blackbox threat model, where the attacker is not aware of the defense, they are relatively ineffective under whitebox threat model, where the attacker has full knowledge of the defense. In this paper, we propose ExAD, a framework to detect adversarial examples using an ensemble of explanation techniques. Each explanation technique in ExAD produces an explanation map identifying the relevance of input variables for the model's classification. For every class in a dataset, the system includes a detector network, corresponding to each explanation technique, which is trained to distinguish between normal and abnormal explanation maps. At test time, if the explanation map of an input is detected as abnormal by any detector model of the classified class, then we consider the input to be an adversarial example. We evaluate our approach using six state-of-the-art adversarial attacks on three image datasets. Our extensive evaluation shows that our mechanism can effectively detect these attacks under blackbox threat model with limited false-positives. Furthermore, we find that our approach achieves promising results in limiting the success rate of whitebox attacks.

==> 03_problem.tex <==
\section{Threat Model}
\label{sec_threat_model}
%\section{Problem Definition}
% \label{sec_problem}
% \subsection{Detecting Adversarial Examples}
% \label{detecting_adversarial_examples}
% Given a DNN classifier $f(\cdot)$ and an input $x$ that is being classified by $f(\cdot)$ as class $C(x) = c$, our goal is to detect if $x$ is a normal example of class $l$ or an adversarial example.
%\subsection{Threat Model}
We assume that the attacker has complete knowledge of the target classifier $f(\cdot)$ including its network architecture, parameters, and training procedure. Depending upon whether the attacker has knowledge of the defense mechanism, we consider two types of threat models. First, we consider \textit{blackbox} attack, where the attacker does not have any knowledge of the defense mechanism. Second, we consider \textit{whitebox} attack, where the attacker has complete knowledge of the defense mechanism including its structure and parameters. For \sysname, this implies that the attacker has full knowledge of the explanation techniques and detector models.
% \begin{itemize}
%     \item \textit{Blackbox attack}: the attacker does not have any knowledge of the defense mechanism.
%     \item \textit{Whitebox attack}: the attacker has complete knowledge of the defense mechanism including its structure and parameters. 
% \end{itemize}

==> 08_availability.tex <==
\section*{Availability}
% The reference code for our work can be found at an anonymous GitHub link \footnote{\url{https://github.com/anonymousresearch1/ExAD}}. After the paper, we will be releasing all source code and data for \sysname{} to enable further research in this area.
The reference code for our whitebox defense can be found at an anonymous GitHub link \footnote{\url{https://github.com/anonymousresearch1/ExAD}}. After the paper, we will further release source code and data for \sysname{} to enable research in building more effective whitebox attacks, and developing appropriate defenses.

==> appen2.tex <==
\section{Similarity in Normal Explanations}
\label{ap_similarity_normal}
Our approach is motivated by the observation that normal examples of a class have visually similar (normal) explanations, which are distinguishable from the (abnormal) explanations of adversarial examples. Figure \ref{fig:intr_of_gen_and_adv} shows an example of the similarity in normal explanations for three image datasets. The first row shows five normal examples from the Coat class of FMNIST dataset. The third row shows normal examples from the Airplane class of CIFAR-10 dataset. The fifth row shows normal examples of class Three from MNIST dataset. The second, fourth, and sixth rows show corresponding explanations for the preceeding row using the IG, LRP, and GBP techniques respectively. We observe that the similarity in normal examples of a class translates to similarity in their explanations. On the other hand, explanations derived from adversarial examples are bound to be closely tied to the original class of their seed images. The differences between the seed class and the target class translates to the distinguishability of abnormal explanations of adversarial examples from normal explanations.
\begin{figure}[h]
  \includegraphics[width=1\linewidth]{figures/intr_of_clean_similar.png}
  \caption{\textbf{Similarity in normal explanations.}}
  \label{fig:intr_of_gen_and_adv}
  \vspace{-5mm}
\end{figure}

\section{Generalizability of \sysname-CNN}
\label{ap_generalizability}
Figure \ref{fig:diff_attack_similar_exp} shows explanation maps produced by the integrated gradients technique for adversarial examples created using different attacks. Rows 1 and 2 show explanation maps for adversarial examples which were created using CW$_\infty$ and BIM attacks respectively. Both attacks come under the $L_\infty$ category. The adversarial examples are targeting the Pullover class and their seed images are taken from the Trouser class of FMNIST dataset. Comparing explanation maps in row 1 and row 2 shows that adversarial examples created using different attacks, under the same category ($L_\infty$ in this case) can result in similar explanation maps. This can also be observed for CIFAR-10 dataset (rows 3-4), where we use two $L_0$ attacks, and MNIST dataset (rows 5-6), where we again use two $L_\infty$ attacks.

\begin{figure}[t]
  \includegraphics[width=0.76\linewidth]{figures/diff_attack_similar_exp.png}
  \caption{\textbf{Similarity in explanation maps of adversarial examples created using different attacks.}}
  \label{fig:diff_attack_similar_exp}
  \vspace{-1mm}
\end{figure}

\section{Implementation Details}
\subsection{Training the Target Models}
\label{ap_train_target}
Table \ref{tab:classifier_arch} shows the architecture of the target models for MNIST, FMNIST, and CIFAR-10 datasets.

%% Architecture of Image Classifiers to be defended [NEW]
\begin{table}[h]
  \centering
  \begin{small}
  \caption{Architecture of the image classifiers to be defended.}
  \label{tab:classifier_arch}
  \scalebox{0.95}{
  \begin{tabular}{P{1.2cm}P{1.1cm}P{1.3cm}P{0.8cm}P{1.3cm}P{0.8cm}}
    \toprule
    \multicolumn{2}{c}{MNIST} &\multicolumn{2}{c}{FMNIST} &\multicolumn{2}{c}{CIFAR-10}\\
    \midrule
     Conv.ReLU &8x8x64 &Conv.ReLU &3x3x32 &Conv.ReLU &3x3x64\\
     Conv.ReLU &6x6x128 &Conv.ReLU &3x3x32 &Conv.ReLU &3x3x128\\
     Conv.ReLU &5x5x128 &MaxPooling &2x2 &AvgPooling &2x2\\
     Softmax &10 &Conv.ReLU &3x3x64 &Conv.ReLU &3x3x128\\
      & &Conv.ReLU &3x3x64 &Conv.ReLU &3x3x256\\
      & &MaxPooling &2x2 &AvgPooling &2x2\\
      & &Dense.ReLU &200 &Conv.ReLU &3x3x256\\
      & &Dense.ReLU &200 &Conv.ReLU &3x3x512\\
      & &Softmax &10 &AvgPooling &2x2\\
      & & & &Conv.ReLU &3x3x10\\
      & & & &Softmax &10\\
    \bottomrule
  \end{tabular}
  }
  \end{small}
\end{table}

Table \ref{tab:classifier_params} shows the training and architecture hyperparameters for the target models of the three datasets. 

% Training and architecture hyperparameters of the image classifiers to be defended
\begin{table}[h]
  \centering
  \small
  \caption{Training and architecture hyperparameters of the image classifiers to be defended}
  \label{tab:classifier_params}
  \begin{tabular}{cccc}
    \toprule
    Hyperparameter &MNIST &FMNIST &CIFAR-10\\
    \midrule
     Learning Rate &0.001 &0.01 &0.001\\
     Optimization Method &Adam &SGD &Adam\\
     Batch Size &128 &128 &256\\
     Epochs &50 &50 &50\\
     %LeakyReLU alpha &- &- &0.2\\
     Padding (Conv layers) &Valid &Valid &Same\\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Training Detector Models of \sysname}
\label{ap_train_exp_based}
Table \ref{tab:arch_intr_based_classifier} shows the architecture and hyperparameters used for \sysname-CNN.

%Architecture of ExAD-CNN
\begin{table}[h]
    \centering
    \small
    \caption{Architecture and hyperparameters of \sysname-CNN}
    \scalebox{0.95}{
    \begin{tabular}{P{1.8cm}P{1.5cm}P{3cm}P{1cm}}
        \toprule
        \multicolumn{2}{c}{Architecture} &\multicolumn{2}{c}{Hyperparameters}\\
        \midrule
        Conv.ReLU &3x3x32 &Learning Rate &0.01\\
        Conv.ReLU &3x3x64 &Optimization Method &Adam\\
        MaxPooling &2x2 &Batch Size &32\\
        
        Conv.ReLU &3x3x128 &Epochs &50\\
        Conv.ReLU &3x3x128 &Padding (Conv layers) &Same\\
        MaxPooling &2x2\\
        
        Dense.ReLU &512\\
        Dense.ReLU &64\\
        Softmax &2\\
        \bottomrule
    \end{tabular}
    }
    \label{tab:arch_intr_based_classifier}
\end{table}

Table \ref{tab:arch_hp_exad_ae} shows the architecture and hyperparameters used for \sysname-AE. For MNIST and FMNIST datasets, $H=W=28$. For CIFAR-10 dataset, $H=W=32$.

%Architecture of ExAD-AE
\begin{table}[h]
    \centering
    \small
    \caption{Architecture and hyperparameters of \sysname-AE}
    \scalebox{0.9}{
    \begin{tabular}{P{1.8cm}P{1.5cm}P{3cm}P{1cm}}
        \toprule
        \multicolumn{2}{c}{Architecture} &\multicolumn{2}{c}{Hyperparameters}\\
        \midrule
        Dense.ReLU &HxW &Learning Rate &$10^{-5}$\\
        Dense.ReLU &400 &Optimization Method &Adam\\
        Dense.ReLU &20 &Batch Size &32\\
        Dense.ReLU &400 &Epochs &100\\
        Dense.ReLU &HxW &\\
        Softmax &2\\
        \bottomrule
    \end{tabular}}
    \label{tab:arch_hp_exad_ae}
\end{table}

\subsection{Performing Whitebox Attack}
\label{ap_whitebox}
Table \ref{tab:hyperparameters_whitebox} shows the hyperparameters for the whitebox attack.

%Hyperparameters of the whitebox attack on explanations
\begin{table}[h]
    \centering
    \small
    \caption{Hyperparameters used in whitebox attack.}
    \begin{tabular}{cccc}
        \toprule
        Method &Iterations &Learning Rate &Factors\\
        \midrule
        LRP &1500 &$10^{-3}$ &2x$10^{-4}$, $10^6$\\
        GBP &1500 &$10^{-3}$ &$10^{11}$, $10^6$\\
        IG &500 &$5x10^{-3}$ &$10^{11}$, $10^6$\\
        PA &1500 &$2x10^{-3}$ &$10^{11}$, $10^6$\\
        GradxInput &1500 &$10^{-3}$ &$10^{11}$, $10^6$\\
        \bottomrule
    \end{tabular}
    \label{tab:hyperparameters_whitebox}
    \vspace{-3mm}
\end{table}

\section{Illustration of Whitebox Attack}
\label{ap_illustration_whitebox}
\begin{figure}[t]
  \includegraphics[width=0.95\linewidth]{figures/whitebox_illustration.png}
  \caption{\textbf{Illustration of whitebox attack.}}
  \label{fig:whitebox_illustration}
\end{figure}

Figure \ref{fig:whitebox_illustration} shows an illustration of our whitebox attack approach, discussed in Section \ref{adaptive_adversaries}. The leftmost image in the first row shows a seed image $x$, which is a normal example from class Airplane of CIFAR-10 dataset. In the first step, we use CW$_\infty$ attack to add perturbations $\delta x$ to $x$, which results in the adversarial example $x' = x + \delta x$. The rightmost image of row 1 shows $x'$. The example $x'$ is misclassified as class Automobile by target model $f(\cdot)$. The second row shows the explanation maps produced for $x'$ by the five techniques. We find that all detector models classify these explanation maps as abnormal. We observe in row 2 that the explanation maps are not consistent with the expected normal explanations of class Automobile. As an adaptive adversary, we now intend to target an explanation technique. For this illustration, we choose to target LRP. To this end, we randomly select an example $x_r$ from class Automobile, for which the explanation map produced by LRP is classified as normal by the corresponding detector model. We show $x_r$ as the first image in row 3. Its explanation map by LRP, shown as the second image in row 2, is set as the target map $h^t_{LRP}$. Then, we perform the optimization for the loss function \ref{wb_opt_eqn} (shown in Section \ref{adaptive_adversaries}) using $x'$ and $h^t_{LRP}$. After the optimization completes, we obtain the final adversarial example $x'' = x' + \delta x'$, which is shown as the rightmost image in row 4. The bottom row shows the explanation maps produced by the five techniques for $x''$. We observe that targeting LRP results in the explanation map produced by LRP (first image in row 5) to be very close to the target map. Also, the explanation maps for GBP (second image in row 5) and PA (fourth image in row 5) are also fairly close to the target map. We find that all three of these explanation maps are classified as normal by their respective detector models. However, we observe that the explanation maps produced by the gradient-based techniques, i.e., IG (third image in row 5) and GTI (rightmost image in row 5), are not as close to the target map. Both these explanation maps are classified as abnormal by their respective detector models. Therefore, using an ensemble of detector models corresponding to diverse explanation techniques, our defense is able to mitigate this whitebox attack by correctly identifying $x''$ as an adversarial example.


\section{Transferability of Whitebox Attacks}
\begin{figure*}[b]
  \includegraphics[width=0.9\textwidth]{figures/transferability_individual_datasets.png}
  \caption{\textbf{Transferability of whitebox attack and detection rate on individual datasets.}}
  \label{fig:whitebox_transferability_individual}
\end{figure*}

Figure \ref{fig:whitebox_transferability_individual} shows results on the transferability of whitebox attack on explanation techniques, as well as the detection rates obtained by our defense, for the three datasets. Previously, we had only shown mean values across datasets in Figure \ref{fig:transferability_all}. 
%In Figure \ref{fig:whitebox_transferability_individual}, the leftmost, middle, and rightmost matrices show results for MNIST, FMNIST, and CIFAR-10 datasets respectively. 
In Figure \ref{fig:whitebox_transferability_individual}, each value shows the mean detection rate for adversarial examples created using different attacks (except while targeting IG technique which only uses CW$_2$ attack) and considering all target classes. On all three datasets, we observe that targeting an explanation technique has a higher impact on detector models corresponding to the other technique(s) of the same kind (gradient-based or propagation-based). 
%On MNIST and FMNIST dataset, targeting LRP was very effective on the LRP-based detector models, as it resulted in 0\% detection rate. 

In terms of impact on \sysname, on all three datasets, targeting gradient-based techniques (IG and GTI) is relatively less effective. For instance, on MNIST, we obtain 100\% detection rate by our approach while targeting IG and GTI techniques. In contrast, we observe that targeting propagation-based techniques is more effective across datasets. On MNIST dataset, the detection rate of the defense on propagation-based techniques is nearly 89\%. On CIFAR-10 dataset, targeting the PA technique results in the lowest detection rate of 80.67\% by \sysname. On FMNIST dataset, the overall performance is fairly consistent while targeting propagation-based techniques. The highest impact is produced by targeting LRP, for which \sysname{} obtains a detection rate of 93.13\%.

\section{Fragility of Explanations}
\label{ap_fragility}
\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\linewidth, scale=0.5]{figures/intr_with_noise.png}
  \caption{ Effect of adding random perturbations, with increasing threshold of $L_\infty$ distance, on explanations by LRP. 
  }
  \label{fig:intr_shirt_with_noise}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.65\linewidth, scale=0.5]{figures/acc_noisy.png}
  \caption{\textbf{Impact of fragility of explanations \cite{ghorbani2019interpretation}.}}
  \label{fig:acc_on_noisy}
\end{figure}

%In Section \ref{subsec_change_expl_not_classif}, we discussed how an attacker may add adversarial perturbations which produce examples that retain the true classification, but have very different explanations~\cite{ghorbani2019interpretation}. 
In Section \ref{subsec_change_expl_not_classif}, we discussed an attack which shows the fragility of explanations~\cite{ghorbani2019interpretation}. Figure \ref{fig:intr_shirt_with_noise} shows an example of this attack for the case of random perturbations. 
The leftmost image in first row is a normal example from the Sneaker class of FMNIST dataset. The next image in first row shows a manipulated image created by adding random perturbations to the normal example such that the prediction remains unchanged, and the perturbations do not exceed a threshold value of 1, in terms of $L_\infty$ distance. The next three images are created in a similar manner but with increased threshold values of 2, 4, and 8 respectively. The second row shows the corresponding explanations produced by LRP technique. We observe that with increased noise threshold, the explanations also become noisy.
With our defense, if such explanations are classified as abnormal, then the corresponding inputs would be considered adversarial (false-positive). Figure \ref{fig:acc_on_noisy} shows that adding random perturbations to normal examples results in a decline of the target classifier's classification accuracy with increasing noise threshold. We discussed in Section \ref{subsec_change_expl_not_classif} that the impact of this attack depends on the nature of the application using the defense. For instance, our approach will not adversely impact applications which consider such perturbed examples as abnormal.

%This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.This is some dummy content.

==> unused.tex <==
\subsection{Explainable Machine Learning}
\label{background:intr_ml}
Our work uses recent advances in explainable machine learning to examine a classification decision and uncover the relevance of different input variables (or pixels). Current explanation techniques can be broadly categorized into two kind of methods. First, 
%which can be divided into the following two categories depending on whether explanation content is generated after or along with model construction.

\subsubsection{Post-hoc Explanation} 
The first category is \textit{post-hoc explanation}. These techniques try to explain the prediction results after the model is built. Typically, for image inputs, the goal is to identify which pixels in an input image are most responsible for the prediction result~\cite{Simonyan-etal13deepInsideCNNsaliency, Selvaraju-etal16gradCAM, Zhou-etal16CAM, Smilkov-etal18smoothgrad, Sundararajan-etal16integratedGradient, Bach-etal15onPixelwise}. The explanation result is often termed as a \textit{saliency map}, or more generally, an \textit{explanation map}. One of the early techniques to generate an explanation map computed the gradients of a target class with respect to the input image~\cite{Simonyan-etal13deepInsideCNNsaliency, baehrens2009explain}. Some variants of this method improve the explanation quality and stability by averaging a group of explanation results sampled around the query point~\cite{Smilkov-etal18smoothgrad}, averaging a series of explanation results along a predefined path in the input space~\cite{Sundararajan-etal16integratedGradient}, or multiplying the feature sensitivity with the feature values~\cite{shrikumar2016not}. 
%Besides, we can also use interpretable model to mimic the behavior of the blackbox model~\cite{Ribe-etal16why, Che-etal15distilling}. 

\subsubsection{Embedded Explanation} The second category is \textit{embedded explanation}, where explainable elements are directly built into models and can provide an explanation along with the prediction result~\cite{Rudin19pleaseStop}. Attention mechanism is a widely applied technique in unveiling the internal information flow towards model prediction~\cite{Velickovic-etal18graphAttention, Luong-etal15attentionTranslation}. Another line of research tries to disentangle the interaction between features to reduce the complexity of understanding how information from input features flow towards the output~\cite{Tsang-etalNIPS18interactionTransparency}.

Our work in this paper does not require explainable elements to be already built into models. We will instead utilize a number of post-hoc explanation techniques which we discuss in Section \ref{gen_of_interpretations}.

%The availability of such interpretation techniques has made it practical to obtain explanations of a classifier's decision-making, such as important attributes of an input that determine its classification. 
% While early works in explainable machine learning focused on producing explanations for image classifiers \cite{Simonyan-etal13deepInsideCNNsaliency}, many recent works have expanded the coverage to other domains, such as LEMNA \cite{guo2018lemna} that provides explanations for the security domain. Moreover, local-explanation based methods, such as LIME \cite{Ribe-etal16why}, can more generally explain any classifier with access to its prediction function. The availability of such explanation techniques ensures that our proposed framework, which relies on interpreting the target model for its defense, can be applied to multiple application areas.
%With the availability of various interpretation techniques, today we can interpret classification decisions of almost any classifier.  

\subsection{Whitebox [old]}
%As an adaptive adversary, we attack target model $f(\cdot)$ to have an example be misclassified as class $c$. The adversary takes a seed image $x$ for performing the attack, such that $C^*(x) \neq c$ and $f(x) \neq c$, where $C^*(x)$ represents the true label and $f(x)$ represents the prediction. As an adaptive adversary, we follow a two-step process towards conducting the attack. First, we attack the target model $f(\cdot)$ as before to generate an adversarial example $x'$. For this step in our experiment, we re-use the adversarial examples created as part of blackbox attack. Recall that under blacbox threat model, the attacker has complete knowledge of the target model. Therefore, these adversarial examples are very likely to be misclassified by $f(\cdot)$. Indeed, as shown in Table \ref{tab:eval_of_blackbox_attacks}, we obtain successful evasion rate of over 85\% for all attacks. However, in this step, as the attacker was assumed to not have knowledge of the defense, these adversarial examples are likely to result in explanation maps which will be considered as abnormal by one or more of the detector models. Using the recent work on attacking an explanation technique \cite{dombrowski2019explanations}, we now introduce an additional step. 


%Such an adaptive adversary can generate adversarial examples that fool the target model into producing desired misclassifications and the targeted explanation technique into producing normal explanation maps. We introduce an extra cross-entropy loss of the interpretation-based model $G(\cdot)$ in the optimization function of the adversary. In this way, these adversarial examples are supposed to fool both the target model and the detector through the adversarial example $x'$ and its interpretation $E(x')$ respectively. But, the interpretation generated using Grad-CAM is not directly differentiable. This increases the difficulty for attackers in explicitly computing the gradients to perform the adaptive attack and is referred to as the problem of obfuscated gradients. To address this concern, we leverage a powerful solution called Backward Pass Differential Approximation (BPDA) to approximate the gradients \cite{athalye2018obfuscated,raff2019barrage}. Specifically, we introduce a neural network with the architecture of U-Net as an interpreter to learn the function that approximates the mapping from the inputs to their interpretations \cite{dabkowski2017real}. As a result, an adaptive adversary can combine the classifier, the interpreter and the detector into a whole model with differentiable gradients which can then be attacked. This results in a powerful adaptive adversary.

%\blue{Finally, we take 1000 examples from each of the three image datasets and construct as many adversarial examples for the adaptive adversary using the $CW_2$ attack with the modified loss function defined above. With this evaluation, we find that the success rate of the attack was limited to 58\% on MNIST dataset, 60\% on FMNIST dataset, and 55\% on CIFAR-10 dataset. If we remove the cross-entropy loss of model $G(\cdot)$ from the attack's optimization, the success rate jumps to 100\% on all three datasets. To the best of our knowledge, we believe that IBD is the first detection mechanism to significantly limit the success rate of whitebox attacks.}


Given a normal image $x \in \Bbb R^d$ with correctly classified class $C(x) = c$ by target model $f(\cdot)$. We follow a two-step process towards conducting a whitebox attack. First, we use a blackbox attack technique to generate an adversarial example $x'$ which is misclassified as $C(x')=t$, where $t$ is the targeted class. Recall that under blackbox threat model, the attacker has complete knowledge of the target model. Therefore, $x'$ is very likely to be misclassified as class $t$. 
%With \sysname-CNN as part of the system, the $j-th$ explanation technique $h_j(\cdot)$ will produce an explanation map $h_j(x')$ for the classification of $x'$ as $t$. 
%%% $g_{c,j}(\cdot)$
With \sysname-CNN as part of the system, each explanation technique will produce an explanation map for the classification of $x'$ as $t$. Here, it is likely that one of the explanation maps may get classified as abnormal by the corresponding detector model, as the attack did not account for the defense. 

==> unused_limitation.tex <==
\section{Limitation}
\label{limitation}
Our detection mechanism and scope of evaluation has certain limitations. First, the neural network based detector model for a class requires instances of abnormal interpretations which are derived from adversarial examples that target that class. We found this detector model to work better for an attack method when adversarial examples generated using that attack method were included in the training process to produce abnormal interpretations. Nevertheless, for an attack method not included in the training process, our findings in Section \ref{experiment_train_limited} showed that the detection rates do not reduce significantly. Second, as discussed in Section \ref{eval_reliability_of_intr}, we do not consider adversarially perturbed examples as normal examples even if they retain their original classification. Finally, our evaluation has only considered targeted attacks, but in future work we plan to extend the evaluation to untargeted adversarial attacks as well. 

==> unused_whitebox.tex <==
\subsection{Evaluation of whitebox attack with adaptive adversaries}
\label{adaptive_adversaries}

% Evaluation of whitebox attack
\begin{table}
  \centering
  %\setlength{\tabcolsep}{1pt}
  \caption{Evaluation of whitebox attacks.}
  \label{tab:eval_of_whitebox_attacks}
  \scalebox{0.85}{
  \begin{tabular}{P{1cm}P{1.6cm}P{2cm}P{1cm}P{1cm}}
  
    \toprule
     &Target Explanation Method &Mean Success Rate without defense &Cost (s) &$L_2$ \newline Distortion\\
     \midrule
      %%%%%%%%%%%%%%%%%%%%%%%% MNIST %%%%%%%%%%%%%%%%%%%%%%%%%
      %%%Linf%%%
      \multirow{5}{*}{\rotatebox[origin=c]{90}{MNIST}} 
        &LRP &99.00\% &137.07 &2.49\\
        &GBP &95.17\% &50.15 &2.64\\
        &IG &82.00\% &506.75 &2.81\\
        &PA &96.17\% &57.74 &2.55\\
        &GTI &91.50\% &48.96 &2.50\\
     \midrule
      %%%%%%%%%%%%%%%%%%%%%%%% FMNIST %%%%%%%%%%%%%%%%%%%%%%%%%
      %%%Linf%%%
      \multirow{5}{*}{\rotatebox[origin=c]{90}{FMNIST}} 
        &LRP &99.17\% &169.36 &2.28\\
        &GBP &95.33\% &51.03 &2.34\\
        &IG &89.00\% &510.47 &2.33\\
        &PA &93.67\% &57.77 &2.76\\
        &GTI &91.50\% &49.12 &2.31\\
     \midrule
      %%%%%%%%%%%%%%%%%%%%%%%% CIFAR10 %%%%%%%%%%%%%%%%%%%%%%%%%
      %%%Linf%%%
      \multirow{5}{*}{\rotatebox[origin=c]{90}{CIFAR-10}} 
        &LRP &99.00\% &138.83 &2.26\\
        &GBP &97.33\% &51.35 &2.24\\
        &IG &94.00\% &484.02 &3.87\\
        &PA &96.00\% &66.53 &3.20\\
        &GTI &95.33\% &66.80 &3.45\\

    \bottomrule
  \end{tabular}}
  \vspace{-3mm}
\end{table}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/transferability_all_datasets.png}
  \caption{\textbf{Transferability of whitebox attack}}
  \label{fig:transferability_all}
  \vspace{-5mm}
\end{figure}

In this section, we evaluate our defense, with the \sysname-CNN setting, under whitebox threat model for an adaptive adversary. Here, we build upon recent research which shows that explanations can be unreliable \cite{kindermans2017reliability} and can be manipulated to produce a target explanation map \cite{zhang2020interpretable, dombrowski2019explanations}. Below, we present our approach to conduct a whitebox attack for generating an adversarial example.

\textbf{Whitebox Attack Approach.}
Given a normal image $x \in \Bbb R^d$ with correctly classified class $C(x) = c$ by target model $f(\cdot)$, we follow a two-step process towards conducting a whitebox attack. First, we use a blackbox attack to generate an adversarial example $x'$ which is misclassified as $C(x')=t$, where $t$ is the targeted class. While $x'$ is likely to fool $f(\cdot)$, it is likely to be correctly classified as an adversarial example by the defense, which has not yet been accounted for by the attack. As a next step, we consider a target explanation technique $h_j(\cdot)$, which produces an explanation map $h_j(x')$ that is correctly classified as abnormal by the corresponding detector model $g_{t,j}(\cdot)$. Our goal in this step is to manipulate $x'$ to create a final adversarial example $x'' = x' + \delta x'$ for which the following properties hold.
\begin{itemize}
    \item The target model's classification remains approximately constant, i.e. $f(x'') \approx f(x')$
    \item The explanation map $h_j(x'')$ is close to a target explanation map $h_j^t$ that is classified as normal by $g_{t,j}(\cdot)$
    \item The norm of the perturbation $\delta x'$ added is small. 
\end{itemize}
 To obtain the target explanation map $h_j^t$, we randomly select a normal example $x_r$ from class $t$ and check if its explanation map $h_j(x_r)$ is classified as normal by $g_{t,j}(\cdot)$. If so, we set the target explanation map as $h_j^t = h_j(x_r)$. Else, we repeat the process until we find such an example. This search is fairly quick because explanation maps of normal examples of a class are very likely to be correctly classified as normal by the detector models. Finally, we generate $x''$ by optimizing the following loss function
\begin{equation}
\label{wb_opt_eqn}
    \mathcal{L} = || h_j(x'') - h_j^t||^2 + \gamma||f(x'') - f(x')||^2
\end{equation}
with respect to $x''$ using gradient descent, such that $\|\delta x'\|_2 < \epsilon$. The first term in the loss function ensures that the explanation map for $x''$ is close to the target map, while the second term ensures the prediction by the target model is still the misclassified class $t$. The weighting of these two terms is controlled by hyperparameter $\gamma \in \Bbb R_+$. 
To compute the gradient with respect to the input $\triangledown h_j(x'')$, we follow the strategy by Dombrowski et al. of replacing relu with the softplus function to circumvent the problem of vanishing second-derivative \cite{dombrowski2019explanations}. A similar strategy of approximating relu was used by Zhang et al.~\cite{zhang2020interpretable}.
% The authors state that computing the gradient with respect to the input $\triangledown h_j(x'')$ is challenging. This is because, for relu-networks such as our target models, the gradient depends on the vanishing second derivative of non-linearities. To overcome this problem, the authors replace the relu with softplus non-linearities
% \begin{equation*}
%     \textnormal{softplus}_{\beta}(x) = \frac{1}{\beta} \textnormal{log} (1 + e^{\beta x})
% \end{equation*}
% For large $\beta$ values, softlus provides an approximation of relu, but has a well-defined second derivative. 
After the optimization completes, we test whether the manipulated image $x''$ fools the original relu-based target model $f(\cdot)$ as well as our defense. We provide an illustration of our approach in Appendix \ref{ap_illustration_whitebox}.

\textbf{Evaluation of Whitebox Attack.}
To perform the first step of the above approach, we re-use the successful adversarial examples $X'$ created using blackbox attacks. While targeting integrated gradients (IG), we only used adversarial examples from CW$_2$ attack as we find targeting IG to incur very high cost. For targeting remaining techniques, we use adversarial examples from all six attacks.
Then, for each adversarial example $x' \in X'$, we perform the second step using the optimization process described above to obtain final adversarial examples $X''$.

Table \ref{tab:eval_of_whitebox_attacks} shows a summary of the whitebox attack. Column 3 shows the mean success rate of the final adversarial examples in retaining the desired misclassification in the target model. The mean is computed over success rates obtained for different attacks (except the IG technique for which we only use CW$_2$ attack). We do not show individual success rates for each attack because they were very similar for any target technique.
In Table \ref{tab:eval_of_whitebox_attacks}, we observe that setting the target as LRP results in the highest success rate, with least $L_2$ distortion. However, as shown in Column 4, the average time required per example to target LRP is over 130 seconds which is quite high compared to targeting GBP, PA, or GTI techniques.

Figure \ref{fig:transferability_all} shows the results of the whitebox attack. 
%The final adversarial examples created using whitebox attack are treated as regular inputs to the system with \sysname{} included as a defense mechanism. 
%For each adversarial example $x''$, \sysname{} classifies it as adversarial if the explanation map produced by any explanation technique is classified as abnormal by the corresponding detector model. 
Each row represents the targeted explanation technique. Columns 1-5 show the detection rate obtained by individual detector models corresponding to the five explanation techniques in correctly classifying explanation maps as abnormal. Column 6 shows the overall performance by \sysname-CNN{} in correctly classifying the examples as adversarial. From Figure \ref{fig:transferability_all}, we make several interesting observations. First, we notice the values along the diagonal (from top-left to bottom-right) are all very low. This is natural as the detector model corresponding to the targeted technique is expected to correctly classify very few explanations as abnormal. For instance, targeting GTI causes its detector model to have a detection rate of only 19.41\%. Second, we observe that targeting a gradient-based technique often results in the detector model corresponding to the other gradient-based technique to also misclassify. For instance, targeting IG results in the GTI-based detector model to have a detection rate of 64.65\%. Similarly, targeting GTI has a noticeable impact on the IG-based detector model. The same phenomenon can be observed for propagation-based techniques (LRP, GBP, and PA). As it follows, we observe that targeting gradient-based techniques have relatively less impact on detector models of propagation-based techniques, and vice-versa. 
%In other words, for an adversarial example produced by targeting a propagation-based technique, it is likely that other propagation-based techniques will produce an explanation map which is close to the target map. However, the explanation maps produced by gradient-based techniques for such examples will be less likely to be close to the target map.
For an adversarial example produced by targeting a certain technique, it is likely that other techniques which share similar underlying mechanisms will produce an explanation map that is close to the target map. However, the explanation maps produced by techniques which aren't as similar are less likely to be close to the target map. 
%The latter observation is consistent with transferability properties  by Zhang et al. \cite{zhang2018detecting} while using a different set of diverse explanation methods.
As shown in Columnn 6 of Figure \ref{fig:transferability_all}, using an ensemble of gradient-based and propagation-based techniques, \sysname{} is able to significantly limit the success rate of whitebox attacks. 
We find \sysname{} to be relatively more robust when gradient-based techniques are targeted. We achieve 99.67\% detection rate for IG as the target, and 98.94\% for GTI as the target. For propagation-based techniques, the highest impact is caused by targeting PA, which results in a detection rate of 88.61\%. For the case of targeting LRP and GBP, we obtain detection rates of 90.11\% and 91.55\%, respectively. We refer to Appendix \ref{ap_transferability} for further analysis on individual datasets.
